Fast Deep Hedging with Second-Order Optimization

Hedging exotic options in presence of market frictions is an important risk management task. Deep hedging can solve such hedging problems by training neural network policies in realistic simulated markets. Training these neural networks may be delicate and suffer from slow convergence, particularly for options with long maturities and complex sensitivities to market parameters. To address this, we propose a second-order optimization scheme for deep hedging. We leverage pathwise differentiability to construct a curvature matrix, which we approximate as block-diagonal and Kronecker-factored to efficiently precondition gradients. We evaluate our method on a challenging and practically important problem: hedging a cliquet option on a stock with stochastic volatility by trading in the spot and vanilla options. We find that our second-order scheme can optimize the policy in 1/4 of the number of steps that standard adaptive moment-based optimization takes.

==> myextdash.tex <==
\newif\ifshortcuts
\newif\ifcyremdash

% Uncomment to enable options manually
\shortcutstrue  % Enable the shortcuts option
%\cyremdashtrue  % Enable the cyremdash option

% Start of pasted content from the .sty file

\makeatletter  % Needed to handle @ in macro names

\def\EXD@test#1{%
  \@ifstar{\let\EXD@break\nobreak #1}{\let\EXD@break\@empty #1}%
}

\DeclareRobustCommand{\Hyphdash}{\EXD@test{\EXD@dash-}}
\DeclareRobustCommand{\Endash}{\EXD@test{\EXD@dash{--}}}
\DeclareRobustCommand{\Emdash}{\EXD@test{\EXD@emd@sh}}
\DeclareRobustCommand{\Halfspace}{\@tempcnta\z@
  \@ifstar{\nobreak\EXD@space\ignorespaces}{\EXD@space\ignorespaces}%
}

\def\EXD@dash#1{%
  \nobreak\leavevmode\hbox{#1}\EXD@break\hskip\z@skip \ignorespaces
}

\def\EXD@emd@sh{%
  \ifvmode
    \EXD@emdash\nobreak\hskip.35em
  \else
    \unskip\nobreak\@tempcnta\m@ne
    \EXD@space \EXD@emdash \EXD@break \EXD@space
  \fi \ignorespaces
}

\def\EXD@space{%
  \edef\@tempa{%
    \ifnum\@tempcnta<\z@ .4\else \ifnum \@tempcnta=\z@ .5\else .6\fi\fi
  }%
  \hskip \@tempa\fontdimen2\font \@plus .5\fontdimen3\font
  \@minus \@tempa\fontdimen4\font
  \@tempcnta -\@tempcnta
}

\def\EXD@emdash{\leavevmode\hbox{---}}

% Handle "shortcuts" option
\ifshortcuts
  \DeclareRobustCommand{\HyphOrDash}{%
    \let\EXD@break\@empty
    \@ifnextchar/{\EXD@d@sh}{%
      \@ifnextchar-{\EXD@hdash}{%
        \@ifnextchar,{\EXD@sp@ce}{\EXD@hyph}%
      }%
    }%
  }
  \DeclareRobustCommand{\BarOrDash}{%
    \let\EXD@break\nobreak
    \@ifnextchar/{\EXD@d@sh}{%
      \@ifnextchar={\EXD@bdash}{%
        \@ifnextchar,{\nobreak\EXD@sp@ce}{\EXD@bar}%
      }%
    }%
  }
  \def\EXD@d@sh/{\EXD@dash-}
  \def\EXD@sp@ce,{\EXD@space}
  \def\EXD@hdash-{\@ifnextchar-{\EXD@hhdash}{\EXD@dash{--}}}
  \def\EXD@bdash={\@ifnextchar={\EXD@bbdash}{\EXD@dash{--}}}
  \def\EXD@hhdash-{\EXD@emd@sh}
  \def\EXD@bbdash={\EXD@emd@sh}
  \AtBeginDocument{%
    \let\EXD@hyph\- \let\@dischyph\HyphOrDash \let\-\@dischyph
    \let\EXD@bar\=  \let\@acciii\BarOrDash    \let\=\@acciii
  }
\fi

% Handle "cyremdash" option
\ifcyremdash
  \def\EXD@emdash{\leavevmode\hb@xt@.8\fontdimen6\font{--\hss--}}
\fi


